Photon emission from quark-gluon plasma out of equilibrium

The photon emission from a non-equilibrium quark-gluon plasma (QGP) is analyzed. We derive an integral equation that describes photon production through quark-antiquark annihilation and quark bremsstrahlung. It includes coherence between different scattering sites, also known as the Landau-Pomeranchuk-Migdal effect. These leading-order processes are studied for the first time together in an out-of-equilibrium field theoretical treatment that enables the inclusion of viscous corrections to the calculation of electromagnetic emission rates. In the special case of an isotropic, viscous, plasma the integral equation only depends on three constants which capture the non-equilibrium nature of the medium.

==> _.tex <==
%% LaTeX2e file `@'
%% generated by the `filecontents' environment
%% from source `paper' on 2017/09/18.
%%
      author         = "Kubo, Ryogo",
      title          = "{Statistical mechanical theory of irreversible processes.
                        1. General theory and simple applications in magnetic and
                        conduction problems}",
      journal        = "J. Phys. Soc. Jap.",
      volume         = "12",
      year           = "1957",
      pages          = "570-586",
      doi            = "10.1143/JPSJ.12.570",
      SLACcitation   = "%%CITATION = JUPSA,12,570;%%"
}
@article{Martin:1959jp,
      author         = "Martin, Paul C. and Schwinger, Julian S.",
      title          = "{Theory of many particle systems. 1.}",
      journal        = "Phys. Rev.",
      volume         = "115",
      year           = "1959",
      pages          = "1342-1373",
      doi            = "10.1103/PhysRev.115.1342",
      SLACcitation   = "%%CITATION = PHRVA,115,1342;%%"
}
@article{Migdal:1956tc,
      author         = "Migdal, Arkady B.",
      title          = "{Bremsstrahlung and pair production in condensed media at
                        high-energies}",
      journal        = "Phys. Rev.",
      volume         = "103",
      year           = "1956",
      pages          = "1811-1820",
      doi            = "10.1103/PhysRev.103.1811",
      SLACcitation   = "%%CITATION = PHRVA,103,1811;%%"
}
@article{Migdal:1955nv,
      author         = "Migdal, Arkady B.",
      title          = "{Quantum kinetic equation for multiple scattering}",
      journal        = "Dokl. Akad. Nauk Ser. Fiz.",
      volume         = "105",
      year           = "1955",
      pages          = "77",
      SLACcitation   = "%%CITATION = DANKA,105,77;%%"
}
@article{Landau:1953um,
      author         = "Landau, L. D. and Pomeranchuk, I.",
      title          = "{Limits of applicability of the theory of bremsstrahlung
                        electrons and pair production at high-energies}",
      journal        = "Dokl. Akad. Nauk Ser. Fiz.",
      volume         = "92",
      year           = "1953",
      pages          = "535-536",
      SLACcitation   = "%%CITATION = DANKA,92,535;%%"
}
@article{Landau:1953gr,
      author         = "Landau, L. D. and Pomeranchuk, I.",
      title          = "{Electron cascade process at very high-energies}",
      journal        = "Dokl. Akad. Nauk Ser. Fiz.",
      volume         = "92",
      year           = "1953",
      pages          = "735-738",
      SLACcitation   = "%%CITATION = DANKA,92,735;%%"
}
@article{Dion:2011pp,
      author         = "Dion, Maxime and Paquet, Jean-Fran\c{c}ois and Schenke, Bjoern
                        and Young, Clint and Jeon, Sangyong and Gale, Charles",
      title          = "{Viscous photons in relativistic heavy ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C84",
      year           = "2011",
      pages          = "064901",
      doi            = "10.1103/PhysRevC.84.064901",
      eprint         = "1109.4405",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1109.4405;%%"
}
@article{Vujanovic:2013jpa,
      author         = "Vujanovic, Gojko and Young, Clint and Schenke, Bjoern and
                        Rapp, Ralf and Jeon, Sangyong and Gale, Charles",
      title          = "{Dilepton emission in high-energy heavy-ion collisions
                        with viscous hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C89",
      year           = "2014",
      number         = "3",
      pages          = "034904",
      doi            = "10.1103/PhysRevC.89.034904",
      eprint         = "1312.0676",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1312.0676;%%"
}
@article{Paquet:2015lta,
      author         = "Paquet, Jean-Fran\c{c}ois and Shen, Chun and Denicol,
                        Gabriel S. and Luzum, Matthew and Schenke, Bjoern and
                        Jeon, Sangyong and Gale, Charles",
      title          = "{Production of photons in relativistic heavy-ion
                        collisions}",
      journal        = "Phys. Rev.",
      volume         = "C93",
      year           = "2016",
      number         = "4",
      pages          = "044906",
      doi            = "10.1103/PhysRevC.93.044906",
      eprint         = "1509.06738",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1509.06738;%%"
}
@article{Heinz:2013th,
      author         = "Heinz, Ulrich and Snellings, Raimond",
      title          = "{Collective flow and viscosity in relativistic heavy-ion
                        collisions}",
      journal        = "Ann. Rev. Nucl. Part. Sci.",
      volume         = "63",
      year           = "2013",
      pages          = "123-151",
      doi            = "10.1146/annurev-nucl-102212-170540",
      eprint         = "1301.2826",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1301.2826;%%"
}
@article{Jacak:2012dx,
      author         = "Jacak, Barbara V. and Muller, Berndt",
      title          = "{The exploration of hot nuclear matter}",
      journal        = "Science",
      volume         = "337",
      year           = "2012",
      pages          = "310-314",
      doi            = "10.1126/science.1215901",
      SLACcitation   = "%%CITATION = SCIEA,337,310;%%"
}
@article{Gale:2013da,
      author         = "Gale, Charles and Jeon, Sangyong and Schenke, Bjoern",
      title          = "{Hydrodynamic Modeling of Heavy-Ion Collisions}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "A28",
      year           = "2013",
      pages          = "1340011",
      doi            = "10.1142/S0217751X13400113",
      eprint         = "1301.5893",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1301.5893;%%"
}
@book{Bellac2011,
      author         = "Bellac, Michel Le",
      title          = "{Thermal Field Theory}",
      publisher      = "Cambridge University Press",
      year           = "2011",
      url            = "http://www.cambridge.org/mw/academic/subjects/physics/theoretical-physics-and-mathematical-physics/thermal-field-theory?format=AR",
      ISBN           = "9780511885068, 9780521654777",
      SLACcitation   = "%%CITATION = INSPIRE-1384874;%%"
}

@article{Chou1984,
      author         = "Chou, Kuang-chao and Su, Zhao-bin and Hao, Bai-lin and
                        Yu, Lu",
      title          = "{Equilibrium and Nonequilibrium Formalisms Made Unified}",
      journal        = "Phys. Rept.",
      volume         = "118",
      year           = "1985",
      pages          = "1",
      doi            = "10.1016/0370-1573(85)90136-X",
      reportNumber   = "AS-ITP-84-021",
      SLACcitation   = "%%CITATION = PRPLC,118,1;%%"
}

@article{Keldysh1964,
      author         = "Keldysh, L. V.",
      title          = "{Diagram technique for nonequilibrium processes}",
      journal        = "Zh. Eksp. Teor. Fiz.",
      volume         = "47",
      year           = "1964",
      pages          = "1515-1527",
      note           = "[Sov. Phys. JETP20,1018(1965)]",
      SLACcitation   = "%%CITATION = ZETFA,47,1515;%%"
}

@article{Calzetta1986,
      author         = "Calzetta, E. and Hu, B. L.",
      title          = "{Nonequilibrium Quantum Fields: Closed Time Path
                        Effective Action, Wigner Function and Boltzmann Equation}",
      journal        = "Phys. Rev.",
      volume         = "D37",
      year           = "1988",
      pages          = "2878",
      doi            = "10.1103/PhysRevD.37.2878",
      reportNumber   = "MDDP-PP-87-104",
      SLACcitation   = "%%CITATION = PHRVA,D37,2878;%%"
}

@article{Blaizot1992,
      author         = "Blaizot, Jean-Paul and Iancu, Edmond",
      title          = "{Kinetic theory and quantum electrodynamics at high
                        temperature}",
      journal        = "Nucl. Phys.",
      volume         = "B390",
      year           = "1993",
      pages          = "589-620",
      doi            = "10.1016/0550-3213(93)90490-G",
      reportNumber   = "SACLAY-SPH-T-92-071",
      SLACcitation   = "%%CITATION = NUPHA,B390,589;%%"
}

@article{Weigert1990,
      author         = "Weigert, Heribert and Heinz, Ulrich W.",
      title          = "{Kinetic Equations for the Quark - Gluon Plasma and Their
                        Semiclassical Expansion}",
      booktitle      = "{Smolenice Hadron Struc.1989:235-241}",
      journal        = "Z. Phys.",
      volume         = "C50",
      year           = "1991",
      pages          = "195-204",
      doi            = "10.1007/BF01474074",
      reportNumber   = "TPR-90-28",
      SLACcitation   = "%%CITATION = ZEPYA,C50,195;%%"
}

@article{Greiner1998,
      author         = "Greiner, Carsten and Leupold, Stefan",
      title          = "{Interpretation and resolution of pinch singularities in
                        nonequilibrium quantum field theory}",
      journal        = "Eur. Phys. J.",
      volume         = "C8",
      year           = "1999",
      pages          = "517-522",
      doi            = "10.1007/s100529901095",
      eprint         = "hep-ph/9804239",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UGI-98-17",
      SLACcitation   = "%%CITATION = HEP-PH/9804239;%%"
}

@article{Aurenche1998,
      author         = "Aurenche, P. and Gelis, F. and Kobes, R. and Zaraket, H.",
      title          = "{Bremsstrahlung and photon production in thermal QCD}",
      journal        = "Phys. Rev.",
      volume         = "D58",
      year           = "1998",
      pages          = "085003",
      doi            = "10.1103/PhysRevD.58.085003",
      eprint         = "hep-ph/9804224",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-678-98, WIN-98-05",
      SLACcitation   = "%%CITATION = HEP-PH/9804224;%%"
}

@article{Arnold2001,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Photon emission from ultrarelativistic plasmas}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2001",
      pages          = "057",
      doi            = "10.1088/1126-6708/2001/11/057",
      eprint         = "hep-ph/0109064",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-01-21",
      SLACcitation   = "%%CITATION = HEP-PH/0109064;%%"
}

@article{Arnold2001b,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Photon emission from quark gluon plasma: Complete
                        leading order results}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2001",
      pages          = "009",
      doi            = "10.1088/1126-6708/2001/12/009",
      eprint         = "hep-ph/0111107",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-01-22",
      SLACcitation   = "%%CITATION = HEP-PH/0111107;%%"
}

@article{Mrowczynski2000,
      author         = "Mrowczynski, Stanislaw and Thoma, Markus H.",
      title          = "{Hard loop approach to anisotropic systems}",
      journal        = "Phys. Rev.",
      volume         = "D62",
      year           = "2000",
      pages          = "036011",
      doi            = "10.1103/PhysRevD.62.036011",
      eprint         = "hep-ph/0001164",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0001164;%%"
}

@article{AMY_eff_kin,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Effective kinetic theory for high temperature gauge
                        theories}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2003",
      pages          = "030",
      doi            = "10.1088/1126-6708/2003/01/030",
      eprint         = "hep-ph/0209353",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0209353;%%"
}

@book{Kapusta2006,
      author         = "Kapusta, J. I. and Gale, Charles",
      title          = "{Finite-temperature field theory: Principles and
                        applications}",
      publisher      = "Cambridge University Press",
      year           = "2011",
      ISBN           = "9780521173223, 9780521820820, 9780511222801",
      SLACcitation   = "%%CITATION = INSPIRE-738588;%%"
}

@article{Serreau2003,
      author         = "Serreau, Julien",
      title          = "{Out-of-equilibrium electromagnetic radiation}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2004",
      pages          = "078",
      doi            = "10.1088/1126-6708/2004/05/078",
      eprint         = "hep-ph/0310051",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "HD-THEP-03-48",
      SLACcitation   = "%%CITATION = HEP-PH/0310051;%%"
}

@article{Wang1998,
      author         = "Wang, Enke and Heinz, Ulrich W.",
      title          = "{A Generalized fluctuation dissipation theorem for
                        nonlinear response functions}",
      journal        = "Phys. Rev.",
      volume         = "D66",
      year           = "2002",
      pages          = "025008",
      doi            = "10.1103/PhysRevD.66.025008",
      eprint         = "hep-th/9809016",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/9809016;%%"
}

@article{Mamo2015,
      author         = "Mamo, Kiminad A. and Yee, Ho-Ung",
      title          = "{Spin polarized photons from an axially charged plasma at
                        weak coupling: Complete leading order}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "6",
      pages          = "065053",
      doi            = "10.1103/PhysRevD.93.065053",
      eprint         = "1512.01316",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "RBRC-1158",
      SLACcitation   = "%%CITATION = ARXIV:1512.01316;%%"
}

@article{Gagnon2006,
      author         = "Gagnon, Jean-Sebastien and Jeon, Sangyong",
      title          = "{Leading order calculation of electric conductivity in
                        hot quantum electrodynamics from diagrammatic methods}",
      journal        = "Phys. Rev.",
      volume         = "D75",
      year           = "2007",
      pages          = "025014",
      doi            = "10.1103/PhysRevD.75.025014, 10.1103/PhysRevD.76.089902",
      note           = "[Erratum: Phys. Rev.D76,089902(2007)]",
      eprint         = "hep-ph/0610235",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0610235;%%"
}

@article{Gagnon2007,
      author         = "Gagnon, Jean-Sebastien and Jeon, Sangyong",
      title          = "{Leading Order Calculation of Shear Viscosity in Hot
                        Quantum Electrodynamics from Diagrammatic Methods}",
      journal        = "Phys. Rev.",
      volume         = "D76",
      year           = "2007",
      pages          = "105019",
      doi            = "10.1103/PhysRevD.76.105019",
      eprint         = "0708.1631",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0708.1631;%%"
}

@article{Aurenche2002,
      author         = "Aurenche, P. and Gelis, F. and Zaraket, H.",
      title          = "{A Simple sum rule for the thermal gluon spectral
                        function and applications}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2002",
      pages          = "043",
      doi            = "10.1088/1126-6708/2002/05/043",
      eprint         = "hep-ph/0204146",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-909-02, LPT-ORSAY-02-27",
      SLACcitation   = "%%CITATION = HEP-PH/0204146;%%"
}

@article{Baier1991,
      author         = "Baier, R. and Nakkagawa, H. and Niegawa, A. and Redlich,
                        K.",
      title          = "{Production rate of hard thermal photons and screening of
                        quark mass singularity}",
      journal        = "Z. Phys.",
      volume         = "C53",
      year           = "1992",
      pages          = "433-438",
      doi            = "10.1007/BF01625902",
      reportNumber   = "BI-TP-91-15",
      SLACcitation   = "%%CITATION = ZEPYA,C53,433;%%"
}

@article{Kapusta1991,
      author         = "Kapusta, Joseph I. and Lichard, P. and Seibert, D.",
      title          = "{High-energy photons from quark - gluon plasma versus hot
                        hadronic gas}",
      journal        = "Phys. Rev.",
      volume         = "D44",
      year           = "1991",
      pages          = "2774-2788",
      doi            = "10.1103/PhysRevD.47.4171, 10.1103/PhysRevD.44.2774",
      note           = "[Erratum: Phys. Rev.D47,4171(1993)]",
      SLACcitation   = "%%CITATION = PHRVA,D44,2774;%%"
}

@article{Baier1997,
      author         = "Baier, R. and Dirks, M. and Redlich, K. and Schiff, D.",
      title          = "{Thermal photon production rate from nonequilibrium
                        quantum field theory}",
      journal        = "Phys. Rev.",
      volume         = "D56",
      year           = "1997",
      pages          = "2548-2554",
      doi            = "10.1103/PhysRevD.56.2548",
      eprint         = "hep-ph/9704262",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BI-TP-97-11, LPTHE-ORSAY-97-15, GSI-PREPRINT-97-22",
      SLACcitation   = "%%CITATION = HEP-PH/9704262;%%"
}

@article{Schenke2006b,
      author         = "Schenke, Bjoern and Strickland, Michael",
      title          = "{Photon production from an anisotropic quark-gluon
                        plasma}",
      journal        = "Phys. Rev.",
      volume         = "D76",
      year           = "2007",
      pages          = "025023",
      doi            = "10.1103/PhysRevD.76.025023",
      eprint         = "hep-ph/0611332",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0611332;%%"
}

@article{Shen2014,
      author         = "Shen, Chun and Paquet, Jean-Fran\c{c}ois and Heinz, Ulrich
                        and Gale, Charles",
      title          = "{Photon Emission from a Momentum Anisotropic Quark-Gluon
                        Plasma}",
      journal        = "Phys. Rev.",
      volume         = "C91",
      year           = "2015",
      number         = "1",
      pages          = "014908",
      doi            = "10.1103/PhysRevC.91.014908",
      eprint         = "1410.3404",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1410.3404;%%"
}

@inproceedings{Hauksson2016,
      author         = "Hauksson, Sigtryggur and Shen, Chun and Jeon, Sangyong
                        and Gale, Charles",
      title          = "{Bulk viscous corrections to photon production in the
                        quark-gluon plasma}",
      booktitle      = "{8th International Conference on Hard and Electromagnetic
                        Probes of High-energy Nuclear Collisions: Hard Probes 2016
                        (HP2016) Wuhan, Hubei, China, September 23-27, 2016}",
      url            = "http://inspirehep.net/record/1504231/files/arXiv:1612.05517.pdf",
      year           = "2016",
      eprint         = "1612.05517",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1612.05517;%%"
}

@article{Aurenche2000,
      author         = "Aurenche, P. and Gelis, F. and Zaraket, H.",
      title          = "{Landau-Pomeranchuk-Migdal effect in thermal field
                        theory}",
      journal        = "Phys. Rev.",
      volume         = "D62",
      year           = "2000",
      pages          = "096012",
      doi            = "10.1103/PhysRevD.62.096012",
      eprint         = "hep-ph/0003326",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-790-00, BNL-NT-00-11",
      SLACcitation   = "%%CITATION = HEP-PH/0003326;%%"
}

@article{Berges2004,
      author         = "Berges, Juergen",
      title          = "{Introduction to nonequilibrium quantum field theory}",
      booktitle      = "{Proceedings, 9th Hadron Physics and 7th Relativistic
                        Aspects of Nuclear Physics (HADRON-RANP 2004): A Joint
                        Meeting on QCD and QGP: Rio de Janeiro, Brazil, March
                        28-April 3, 2004}",
      journal        = "AIP Conf. Proc.",
      volume         = "739",
      year           = "2005",
      pages          = "3-62",
      doi            = "10.1063/1.1843591",
      note           = "[,3(2004)]",
      eprint         = "hep-ph/0409233",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0409233;%%"
}

@article{Pal2007,
      author         = "Pal, Palash B.",
      title          = "{Representation-independent manipulations with Dirac
                        spinors}",
      year           = "2007",
      eprint         = "physics/0703214",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ed-ph",
      SLACcitation   = "%%CITATION = PHYSICS/0703214;%%"
}

@article{Jeon1994,
      author         = "Jeon, Sangyong",
      title          = "{Hydrodynamic transport coefficients in relativistic
                        scalar field theory}",
      journal        = "Phys. Rev.",
      volume         = "D52",
      year           = "1995",
      pages          = "3591-3642",
      doi            = "10.1103/PhysRevD.52.3591",
      eprint         = "hep-ph/9409250",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-94-09",
      SLACcitation   = "%%CITATION = HEP-PH/9409250;%%"
}

@article{Nopoush2017,
      author         = "Nopoush, Mohammad and Guo, Yun and Strickland, Michael",
      title          = "{The static hard-loop gluon propagator to all orders in
                        anisotropy}",
      year           = "2017",
      eprint         = "1706.08091",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.08091;%%"
}

@article{Mrowczynski2016,
      author         = "Mrowczynski, Stanislaw and Schenke, Bjoern and
                        Strickland, Michael",
      title          = "{Color instabilities in the quark–gluon plasma}",
      journal        = "Phys. Rept.",
      volume         = "682",
      year           = "2017",
      pages          = "1-97",
      doi            = "10.1016/j.physrep.2017.03.003",
      eprint         = "1603.08946",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1603.08946;%%"
}


